Randomized Algorithms for Symmetric Nonnegative Matrix Factorization

Symmetric Nonnegative Matrix Factorization (SymNMF) is a technique in data analysis and machine learning that approximates a symmetric matrix with a product of a nonnegative, low-rank matrix and its transpose. To design faster and more scalable algorithms for SymNMF we develop two randomized algorithms for its computation. The first algorithm uses randomized matrix sketching to compute an initial low-rank approximation to the input matrix and proceeds to rapidly compute a SymNMF of the approximation. The second algorithm uses randomized leverage score sampling to approximately solve constrained least squares problems. Many successful methods for SymNMF rely on (approximately) solving sequences of constrained least squares problems. We prove theoretically that leverage score sampling can approximately solve nonnegative least squares problems to a chosen accuracy with high probability. Additionally, we prove sampling complexity results for previously proposed hybrid sampling techniques which deterministically include high leverage score rows. This hybrid scheme is crucial for obtaining speeds ups in practice. Finally we demonstrate that both methods work well in practice by applying them to graph clustering tasks on large real world data sets. These experiments show that our methods approximately maintain solution quality and achieve significant speed ups for both large dense and large sparse problems.

==> Deterministic_and_Hybrid_LeverageScore_Theory.tex <==
\section{Analysis of Deterministic and Hybrid Leverage Score Sampling for Least Squares}

\subsection{Deterministic Leverage Score Sampling for Least Squares Problems}
Deterministically selecting the coordinates of columns or rows with the highest leverage scores has been explored for the Column Subset Selection Problem \cite{det_samp_levscores}.
The deterministic sampling matrix, which we denote as $\M{S}_\theta$ and is $s_\theta \times m$, is given as 
\begin{equation}
    (\M{S}_\theta)_{ij} = \begin{cases}
        1 \ \text{if row $j$ is the $i$th sample} \\
        0 \ \text{otherwise}
    \end{cases}
\end{equation}
This problem is related to but different from using leverage scores for randomized Least Squares.
We analyze, theoretically, the viability of using deterministic leverage scores sampling for Least Squares problems.
Our main result is presented via Theorem \ref{thm:det_sampling}.
\begin{theorem}
\label{thm:det_sampling}
    Given an overdetermined Least Squares problem defined with full column rank matrix $\M{A}\in \mathbb{R}^{m\times k}$ and $\V{b}\in\mathbb{R}^m$ if the deterministic sampling matrix $\M{S}_\theta$ satisfies $\| \M{S}_\theta\M{U} \|_F^2 = \theta$ such that $1 > k - \theta \ge 0$ and $\V{v} = \min_{\V{x}'}\| \M{S}_\theta(\M{A}\V{x}' - \V{b}) \|$ then
    \begin{equation}
    \label{eq:det_samp_LS}
    \| \M{A}\V{v}- \V{b} \|_F^2 
    \le ( 1+\epsilon) \min_{\V{x}'}\| \M{A}\V{x}' - \V{b} \| 
\end{equation}
where $\epsilon = \frac{\xi}{(1-\xi)^2}$ and $\xi = k - \theta$. 
\end{theorem}
This theorem shows that under the right circumstances deterministic leverage score sampling can work for Least Squares problems.
In \cite{det_samp_levscores} it was shown that if the leverage scores of $\M{A}$ follow certain power-law distributions the constraint that $\xi < 1$ holds.
While this constraint appears to be reasonable in the context of the Column Subset Selection Problem, it maybe not be viable for Least Squares problems.
As $k$ increases we need that $\theta$ remain large enough so that $\xi < 1$.

\subsection{Hybrid Leverage Score Sampling for Least Squares Problems}
A Hybrid scheme for Leverage Score sampling was proposed in \cite{lev_scores4_CP}.
The authors showed that hybrid sampling could drastically improve the convergence rate of the CP decomposition via Alternating Least Squares for large sparse tensors.
In this hybrid sampling method every row with a leverage score higher than a given threshold $1 \ge \tau > 0$ is deterministically sampled and the remaining rows are randomly sampled as normal.
The Hybrid Sampling matrix takes the form
\begin{equation*}
    \M{S}_H  
    = \begin{bmatrix}
    \M{S}_D & \M{0}_{m-s_D\times m-s_D} \\
    \M{0}_{s_R\times s_D} & \M{S}_R
    \end{bmatrix}
\end{equation*}
where $\M{S}_H$ is $s_H \times m$, $\M{S}_D$ is $s_D \times m-s_D$, and $\M{S}_R$ is $s_R \times m - s_D$.

%\kh{This theorem is a place holder and gives the general idea of what we are trying to prove. I think there are some issues with it. First the $1-\delta$ probability might not be quite correct, there might be a half factor missing or something. The constants for $s_R$ might need to be tuned better and re-checked. The role of $\beta$ need to be more carefully checked in how it relates to the deterministic sampling.}
\begin{theorem}
\label{thm:hybrid_sampling}
    Given an overdetermined Least Squares problem defined with full column rank matrix $\M{A}\in \mathbb{R}^{m\times k}$ with economy SVD $\M{A} = \M{U}\M{\Sigma}\M{V}^\Tra$ and $\V{b}\in\mathbb{R}^m$ construct the hybrid sampling matrix $\M{S}_H$ such that $\M{S}_D$ satisfies $\| \M{S}_D\M{U}_D \|_F^2 = k - \xi = \theta$ and $\M{S}_R$ is a random sampling matrix that samples $s_R \ge \xi\max\Big( \frac{1}{\epsilon \delta}, \frac{4}{3(1-\sqrt{2})^2} \ln(\frac{k}{\delta}) \Big)$, and $\V{v} = \min_{\V{x}'}\| \M{S}_H(\M{A}\V{x}' - \V{b}) \|$ then with probability $1-\delta$
    \begin{equation}
    \label{eq:det_samp_LS}
    \| \M{A}\V{v}- \V{b} \|_F^2 
    \le ( 1+\epsilon) \min_{\V{x}'}\| \M{A}\V{x}' - \V{b} \| 
\end{equation}
\end{theorem}


==> Meta_Comments.tex <==
\section{Meta-Comments}
This is a space for discussion of the paper.
Section \ref{SS_discussion} seems to be solid for now.
There is a lot of good stuff with the paper but also a lot that still needs to be done.
I want to list a number of questions that we can answer and what our options are for each of them.

\kh{Contributions list:
\begin{enumerate}
    \item Discussion of the use of complex values in graph clustering.
    \item Run time decrease and large performance boon from using the SVD for Curugingu's algorithm.
    \item Improved result on the Complete Meta-Graph for the DSBM by Cucuringu using a search Heuristic
    \item A relaxation argument for justifying why the algorithm might results in large Imbalanced Cuts.
    \item Results on the Florida Bay Food Web and possibly other food webs.
    \item 
\end{enumerate}
To do list:
\begin{itemize}
    \item Discussion of connectivity needs to be decided. More feeback on this, section 6.
    \item Update the FBFW table, progress made
    \item Abstract needs to be finalized, progress made
    \item Finish secondary foodweb section, progress made
    \item Add Laenen's Algorithm discussion. I put a mention of this in the experiments section. progress made
    \item See note in 4.2.2 on real and imaginary parts of $\M{W}$. 
\end{itemize}
}
\kh{Discussion of other complex Laplacians
\begin{itemize}
    \item Other Complex Laplacians exist
    \item We are focusing on these Laplacians in the context of clustering directed graphs only, not their general utility. (E.g to Graph Neural Networks)
    \item Magnetic Laplacian is a generalization of the Laplacian that we consider. But its still unclear how to choose the parameters of the Magnetic Laplacian.
    \item Is Magnetic Laplacian a generalization of Mohars or the other way around. What about Laenen's Laplacian.
    \item What about the splitting of the imaginary vs complex portions of these Laplacians.
\end{itemize}}

%\sa{On notation: I think the addition of the notation table is welcome. The notation itself seems fine, except for using $\epsilon$ and $\nu$ to denote the number of edges and vertices. I understand the logic (these look like the lowercase versions of $E$ and $V$) but epsilon already has deep connotations in math that no one would associate with ``number of edges" and so this would stick out to many readers as weird and confusing. People almost always just use $m$ and $n$ to denote the number of edges/vertices in a graph (or $|E|$ and $|V|$, although this is more clunky). I understand $m$ and $n$ are already used when defining certain general linear algebra definitions/results, but I doubt slightly ``overloading" these letters will confuse anyone. It is clear (or can be easily made clear) from context when we mean $m$ and $n$ in a generic sense (e.g. in a theorem/definition statement like ``this is an $m \times n$ matrix" or whether we're referring to number of vertices/edges.}

==> Paper_Outline.tex <==
\section{Paper Outline}
\kh{This section for outlining the various sections of the paper and the major points in each section.
Everyone has a text color macro to comment and it is your two initials, for example Grey's is $*backslash*gb$}
\gb{Grey's macro}
\hp{Haesun's macro}
\sa{Sinan's macro}

\paragraph{Grey's outline proposal}
\begin{itemize}
    \item Thesis : we want to developed randomized methods for Symmetric NMF
    \item To this end we discuss and categorize some of the existing randomized methods for regular NMF.
    \item We propose two natural extensions of these methods for SymNMF.
    \item LAI-NMF is a natural way to extend existing randomized compression based techniques to SymNMF.
    \item Leverage Score sampling is a natural extension from the sparse CP decomposition literature.
\end{itemize}

\paragraph{TODO's}
\begin{itemize}
    \item Add pure leverage score sampling data to the the MOG data set.
    \item Add per iteration break down data 
    \item Add top words per group visualization
    \item Re-write Dense section as modified Compressed NMF method.
    \item Re-write Lev-NMF method section
    \item Lesser TODO's:
    \begin{itemize}
        \item Pixel graph plots
        \item FMNIST comparison plot
        \item 
    \end{itemize}
\end{itemize}

==> Reviewer_Responses.tex <==
\newpage
\section{Reviewer Responses}
We thank the referees for their thoughtful and helpful reviews.
As authors we are glad to see mostly positive reviews regarding the high level contributions of the submitted manuscript.
We have carefully read and endeavored to address all comments.
Many of the changes we have added are marked in red text, particularly those that are text based and/or embedded in existing sections.
Larger changes that are not marked in red include
\begin{itemize}
    \item the addition of \Cref{sec:lvs_nls_thm}, which moves the statement of the leverage score sampling theorem to earlier in the paper as suggested;
    \item the addition of \Cref{sec:lvs_sampling_plts}, which includes plots showing some statistics concerning the hybrid sampling method's use in the OAG data set;
    \item changes to \Cref{sec:apx_errors_4LAINMF}, which are primarily moving statements of theorems we use from the Appendix to the main body of the text as suggested.
\end{itemize}

\subsection*{Reviewer 1}
\subsubsection{Main Comments}
\begin{enumerate}
    \item \textbf{Lines 456, 493: The hybrid sampling method was proposed in [31] not [32].}
    Fixed.
    \item \textbf{Lemma 4.3: This result should hold for any choice of rows to include deterministically; it does not have to be those above a given threshold. The result then provides a nice additional justification for why we would want to deterministically include the high leverage score rows: we want to maximize the proportion of the leverage score mass that is included deterministically.} 
    This is a good point. We have added a discussion paragraph to the end of \Cref{sec:hybrid_samp_theory}. We point out that the deterministic row inclusion set $\mathscr{I}_D$ can be determined by any method desired.
    \item \textbf{Line 614-617: This discussion of $\M{X}_j$ and $\M{X}$ is confusingly worded. It would make more sense to define q as a random variable first with a distribution $\tilde{\pi}$. Currently the quantity $\frac{1}{\tilde{\pi}}\V{q}\V{q}^\Tra$ is not clearly defined.} We restructured the discussion as suggested: now $\V{q}$ is defined first along with $\tilde{\pi}$, and $\M{X}$ is defined in terms of $\V{q}$ and $\tilde{\pi}$.
    \item \textbf{Line 672 - 675: When you say you only need $\xi \phi$ samples rather than $k\phi$ samples, this only includes $s_R$. I recommend emphasizing here that the total number of samples is $s_D$ + $\xi\phi$, i.e. that you need to be careful about how many rows you deterministically include.} 
    This is also a good point, we have included new text making this clearer and generally discussing the sample complexity trade offs in more detail.
    \item \textbf{Line 721-723: “Note that we do not report results for LvS-SymNMF on this dataset as the code took prohibitively long to execute.” Can you comment on what part of the LvS- SymNMF ends up being too computationally expensive? Given the laptop setup used for these experiments, what would be approximately the largest size of matrix that you could run LvS-SymNMF?} 
    In our computational set up it takes about 8 seconds to copy a submatrix of the WoS data set consisting of around 5000 row samples.
    (Note that we take column samples of a column major symmetric matrix for efficiency. If you sample against the grain it takes even longer.)
    Even if the LvS-SymNMF method only took 30 iterations, which is the lowest of any method on the WoS data set (see \Cref{tab:WoS_symnmf_exp}), this would result in $2\times30\times8 = 480$ seconds just to perform these operations.
    The factor of 2 comes from the fact that two subproblems are solved for at each iteration.
    We have added a brief discussion of this in \cref{sec:experiments} and emphasized it in the Conclusion.
    \item \textbf{Lines 724-731: “Plots showing the projected gradient values for each algorithm can be found in Appendix C.2...Finally, Appendix C.2 includes plots and tables showing that the use of Algorithm Ada-RRF provides better overall results than using a static choice of q = 2 with IR.” Appendix C.2 seems like the wrong reference for this, and it’s unclear which plots these statements are referring to.} 
    We have fixed this issue and these references now point to the correct figures in \Cref{sec:additional_wos_exps} and we have added more textual discussion of why we think this is a reasonable conclusion.
    \item \textbf{Fig. 1: Does “Comp” stand for compressed? Do the plots for the LAI and compressed algorithms include the time to calculate the low-rank approximate input, i.e. this is occurring during the first approximately 10 seconds?} 
    We have added a paragraph in \Cref{sec:experiments} explaining the naming conventions we use for the legends in the figures. We have also added a line explicitly saying that the plots include the time needed to compute the low-rank approximate input and that this is why the randomized methods appear to `start' later (around the first 10 second or so).
    \item \textbf{Fig. 2: Given that OAG is a dataset for which the LAI method does poorly, I would like to see more discussion of how practitioners should chose between the two algorithms. In the conclusion, the authors say “the Algorithm LAI-SymNMF method is appropriate when a high quality LAI can be computed quickly and captures the underlying NMF signal. In other cases Algorithm LvS-SymNMF can be used.” Would you typically recommend trying LAI first?} 
    We have added more discussion of this, particularly in the Conclusion. We have shied away from making general recommendations in the paper based on the only results appearing here. However it is our opinion that the LAI method is likely suitable for all but large, hypersparse problems. In the Conclusion we have attempted to discuss the trade offs between the two proposed methods in more detail.
    \item \textbf{Fig. 2: I find it intriguing that the OAG problem displays such a strong difference with and without hybrid sampling. I’d like to see further investigation by plotting the percent of samples that are deterministic and the proportion of the leverage score “mass” in the deterministic samples across iterations (akin to Fig. 3 in [31]). If the problem has a relatively small number of high leverage score rows that are being included deterministically, this would match nicely with the analysis of hybrid sampling done by the authors.}
    We have added \Cref{fig:percent_det_samps,fig:percent_lvs} to \cref{sec:moag_appendix} along with a discussion to address this issue. These results show that the leverage score mass becomes concentrated in the small well-defined clusters as the algorithm nears convergence. This confirms the reviewers suspicion that there are a small number of high leverage score rows being deterministically included. 
    \item \textbf{Fig. 4, Tables 4 and 5: There are many algorithms labelled “LRA” instead of “LAI.” I would guess this was an earlier acronym (low-rank approximation) that was changed to LAI (low- rank approximate input). If so, these should be changed to match the main text; otherwise what does LRA stand for?} 
    Yes LRA is supposed to be LAI for the stated reason. This has been fixed.
    \item \textbf{Theorem H.2 should cite the original paper (Drineas, Kannan, and Mahoney; 2006).} 
    Done.
\end{enumerate}

\subsubsection{Suggestions to Improve Clarity}
\begin{enumerate}
    \item \textbf{I did not find the acronym BPP defined in the paper. I suggest defining this acronym when it first appears in Line 281 for clarity.} 
    Added when ANLS is discussed in \Cref{sec:sym_anls}.
    \item \textbf{I would recommend including a reference to Appendix G for the Update() function in the pseudocode for LAI-SymNMF and LvS-SymNMF. The pointer to the appendix is very clear in the main text, but when I was initially skimming the algorithms in the paper, this function definition was unclear.}
    Done.
    \item \textbf{Lemma 4.2: As stated in [9], equation 4.11 is simply the result of the characterization of a global minima of a differentiable function on a convex set, i.e. $\nabla f(\V{x}^*)^\Tra (\V{x} - \V{x}^{*}) \ge 0, \forall \V{x} \in C$ if and only if $\V{x}^{*}$ is the global minimum over a convex set $C$. The fact that we are considering a quadratic program and its perturbation only comes in when evaluating the gradients. Making this clearer would make the lemma more straightforward to parse.} 
    We have added some text emphasizing this point right before \Cref{lem:daneils_qp_ineq}.
    \item \textbf{Line 474, 483, 595,...: The term “deterministically sampled” can be confusing because there is no randomness here; “deterministically included” is clearer.} 
    Done.
    \item \textbf{Line 882: “affect” should be ”effect.”} 
    Done.
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Reviewer 2}
\begin{enumerate}
    \item \textbf{There is some confusion and a few missing references about the HALS algorithm, Section 2.1.2. To provide some background, there are two existing algorithms named HALS to compute solutions to NMF:
    \begin{enumerate}
        \item the work by Cichocki and Phan in 2009 (refs below), where, similarly to ref [56], the rank-one terms $(\V{w}_i, \V{h}_i)$ are updated in sequence for each i.
        \item the work of Gillis and Glineur in 2012 where, similarly to what is proposed in this manuscript, the columns of factors e.g. ($\V{h}_i$) are updated sequentially while fixing $\M{W}$, and vice-versa.
    \end{enumerate}
    The proposed approach in this work is therefore not new. Gillis and Glineur already point out that one can save up some computation time by pre-computing WtW and WtX to update H, and in fact go further by suggesting repeating the updates of H several times before switching to W. This is what I would consider as the default HALS algorithm for NMF, and is a form of inexact ANLS.
    Finally the extension of HALS to l2 squared regularization is simple and known by expert users. It was used for instance in Cohen and Bro 2017 for nonnegative Parafac2.} 
    We have changed the wording when we introduce the HALS update rule we use in \Cref{sec:hals_4symnmf} and have added these citations in appropriate places. We now say that this rule is a combination of the update order used by Gillis and Glineur 2012 and the extension to handle regularization, as done by Cohen and Bro 2017. Since the update rule is very important for obtaining good performance in the leverage score sampling method we think it is important to include and highlight.
    \item \textbf{About the low-rank approximate input method, one of its disadvantages is that while the products WtX and XHt are cheaper to compute, the Gram matrices WtW and HHt are still required in full. This means that in cases where the rank k is not much smaller than one of the dimensions, a significant part of the computational load is not alleviated. I don't think this point is addressed properly in the manuscript. It could be better discussed in terms of limitation of the LAI-NMF approach, and possibly tested in the experiment section (e.g. how much the speed-up offered by LAI-NMF suffers when the rank increases).}
    We have emphasized the point about the Gram matrices in the Conclusion. In fact both randomized methods require a Gram computation of the factors, this can certainly be seen as a hard `lower-bound' on the computation needed by both of the proposed methods. That is for the LvS approach we compute the Grams of the factor matrices to determine exact leverage scores (via Cholesky QR). Even if this step is avoided performing the Update() requires a $O(mk^2)$ computation. As for increasing values of $k$ in our experiments, the value of $k$ that is chosen is determined by the experimental set up (e.g. number of clusters) and so it does not seem appropriate to vary in those contexts.
    \item \textbf{Another remark about LAI-NMF: I believe this technique has already been well-investigated outside the domain of SymNMF. For instance, Vervilet and co-authors in 2019 proposed to compress an input tensor before any tensor decomposition, extending the CANDELINC model. Randomized extensions of HOSVD have been discussed to this end e.g. in Ahmadi-Asl and co-authors in 2021. The authors reference the work of Erichson and co-authors in 2016 about randomized NMF, and while it applies to NMF instead of SymNMF, it is still a very close proposition. Overall I believe most of the novelty in the manuscript is rather located in the sampling approach.}
    We agree that methods similar to this have been well investigated in other contexts, such as tensor decompositions. To this end we cite a number of papers [50,53,58,18,19] and we have added the recommended citations. Additionally, in the Appendix and experiments for WoS dataset we make direct comparisons to Compressed-NMF \cite{Comp_NMF2016}.
    %However these referenced papers do not include experiments or efficient algorithms for preprocessing (Ada-RRF) or post processing (Iterative Refinement) as far as we can tell. It is our belief that our discussion of LAI-SymNMF is more comprehensive both theoretically and in terms of practical implementation than existing methods. 
\end{enumerate}

\subsubsection{Other small remarks}
\begin{enumerate}
    \item \textbf{Authors list: there is a spurious space between Ballard and the symbol.} Fixed.
    \item \textbf{I am not familiar with the notation $R_{\geq 0}$, it seems more common to me to use $R_{+}$?} Changed.
    \item \textbf{There should be a typo in equations (3.3) and (3.4), the $\M{W}_+$ and $\M{H}_+$ symbols have not been introduced before and should probably be $\M{W}^{*}$ and $\M{H}^{*}$?} 
    We do not believe there is a typo here, both sets of factor matrices, with the $+$ and $-$ are defined either in \Cref{lem:lra_nmf_bnd} or in the proof of it.
    \item \textbf{Lines 450-452 The sentence ``sampling does not generally affect the cost of the NLS solve' is misleading. I guess the authors mean that the general formula to compute the cost of NLS given input sizes is unchanged, but at the end of the day, the computational cost will change when using sampling.} 
    We have changed the wording here to refer to the Update() function instead of the NLS problem. The usage of NLS here was erroneous and imprecise.
    \item \textbf{Line 547 ``Equation (4.10) can be interpreted as a perturbed version of Equation (4.9)" is quite imprecise. Not sure what an approximation of an Equation is.} 
    We have changed the language here to refer to objective functions. 
    \item \textbf{Experimental results: generally speaking, it would have helped me understand the experiments better if the methods compared were explicitly listed early on instead of on the fly. This also holds for the general hypotheses tested in the experiments. Some details are also too fuzzy, such as the initialization methods or the clustering strategy (references are provided, but adding a name or a one-sentence explanation avoids having to parse another whole paper for this information).} 
    We have provided additional, high-level descriptions of the clustering strategy cited, as well as the initialization method at the start of \Cref{sec:experiments}. We have added some paragraphs describing the naming convention and the algorithms compared. 
    \item \textbf{Table 2 caption: Tim $\rightarrow$ Time.} Done
    \item \textbf{The references should be checked, there are issues with the HTML addresses, and with capitalization.} Thank you for noticing this. We've tried to catch all instances where capitalization was necessary (e.g. NMF) as well as remove the duplicated addresses and generally cleaning up the references.
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Reviewer 3}
\subsubsection{Major Comments}
\begin{enumerate}
    \item \textbf{There are multiple instances of theoretical results which do not stand alone and require parameter definitions that are not easily found and not referenced. I try to point out all instances of this situation I have identified below in the minor comments/questions section, but I encourage the authors to read through the paper and ensure that all theoretical results either stand alone (include all required parameter definitions) or refer to the required definitions elsewhere.}
    We have attempted to address this issue and reorganized much of the Appendix and some parts of the paper to do so. Hopefully the theoretical results are now more self contained and easier to follow. More specifically we believe that much of the confusion was caused by certain reference theorems being located in the appendix. Many of these have been moved to the main body of the paper as is suggested by the reviewers. This applies mostly to the LAI error bounds. The second source of confusion might be the frequent use of $\delta$ and the various $\epsilon$'s which are both values between 0 and 1. These values are used in many of the theorem and can be thought of as `user input' or more mathematically that the theorem holds for any choice of these parameters. We have reworded some of the theorems to make this clearer and added a footnote to \Cref{thm:nls_bnd}.
    \item \textbf{I think that Section 4.3.1 is of general interest and I recommend considering highlighting this section or its main result Theorem 4.1 by moving them earlier in the paper. Further, can this result be written more generally for general quadratic programs and a broader class of sketches that satisfy the structural conditions? Even if you do not generalize this result, I would recommend commenting on whether other programs would be of interest here and if there are other sketching matrices that satisfy the structural conditions.}
    We have added a discussion after the proof of \Cref{thm:nls_bnd} that addresses some of these questions such as if other sketches are applicable. 
    \item \textbf{The order of the appendix sections is confusing. Proposition A.1 refers to parameters $C_\delta$, $k$ and $q$, which are only defined in the statement of Theorem H.5. Why not place Appendix H before Appendix A, or better yet, include Theorem H.5 in Appendix A.1? I would consider breaking Appendix H up and including these one-off results near where they are used. This way, you prevent confusion and the parameters are more clearly defined for the reader. In fact, Proposition A.1 and Theorem H.5 are so short, I would consider moving them into the main body of the paper in Section 3.4.} We have reorganized the appendix and moved many of these reference theorems into the main body of the paper where they are used. Hopefully this will improve readability. 
\end{enumerate}

\subsubsection{Minor Comments}
\begin{enumerate}
    \item \textbf{Algorithm LAI-SymNMF: In line 3, the comment says “Obtain approximate basis for range of $\M{X}$, $\M{U}$ and $\M{T}$” – I’m not sure why the reference to T here. As it is not defined in this pseudocode, I found it confusing.} Fixed. This was leftover from a previous notation.
    \item \textbf{Section 3.2: You say that you “adapt” Proposition 1 from [54] to your needs. Can you be more specific here so it is clear how your result is different from that of [54]?} 
    Changed the wording to "we can use" instead of adapt. We are combining Proposition 1 from [58] with bounds from the RRF by Gu [25] to obtain the Lemma in Appendix A.1. The `new' \Cref{prop:rndlia_nmf_bnd} is a straightforward combination of existing tools, however the combinations are new and informative.
    \item \textbf{Line 430: “... OLS problem with a many RHS vectors...”} 
    Fixed.
    \item \textbf{Line 491: Remove extra space between “questions” and colon.} 
    Fixed.
    \item \textbf{In Theorem 4.1, what are the parameters $r$, $\epsilon_r$, and $\delta$? These seem to be associated with the leverage score sampling matrix $\M{S}$, but these values do not appear in your definition of $\M{S}$ in eq. (2.11).}
    We have added a footnote and changed the phrasing of the Theorem to make it more clear.
    \item \textbf{Proof of Theorem 4.1: In line 561, shouldn’t this be $\sigma^2 (\M{S}\M{U}_{A})$? If so, I think this will change slightly the application of the first structural condition and the overall result.} 
    Fixed.  The reviewer is correct that it should be the square of the smallest singular value here and for the rest of the proof.  It doesn't change the final result because the first structural condition also bounds the squares of the singular values.
    \item \textbf{Proof of Theorem 4.1: The arrow notation is very informal – replace with words to indicate the conclusions and logic applied.} Agreed. We have replaced the ``implies" arrow notation with words. 
    \item \textbf{Proof of Theorem 4.1: I was confused initially by the absence of $\|\V{z}\|_2$ in line 581. I think it would be more clear if you canceled $\|\V{z}\|_2$ from each side in line 571.} 
    We have rearranged much of this proof to try and make it easier to follow.
    \item \textbf{Proof of Theorem 4.1: $\V{r}_{cls}$ should be $\V{r}_{nls}$} 
    Done.
    \item \textbf{Proposition A.1, Theorem H.5, and possibly elsewhere: You should define more clearly the notation $\sigma_i$. I suppose this is the ith largest singular value, but you have not stated this as far as I can tell. Additionally, which matrix’s singular values are you referring to here? Presumably $\M{X}$, but for an inexperienced reader, this will be confusing.} We have added this notation to the table at the start of the paper.
    \item \textbf{Line 684: Can you give some brief intuition about the initialization strategy applied so that the reader does not need to read the referenced paper?}
    We have added this to \Cref{sec:experiments}.
    \item \textbf{Table 2: Should the “LIA-...” be ”LAI-...”?} 
    Yes, fixed.
    \item \textbf{Table 2 caption: “Tim” should be “Time”} 
    Done.
    \item \textbf{Section 5.1.1: How long do the spectral clustering runs take on average? I think this would be a helpful computational baseline to compare to.}
    The answer is about 35 seconds. This makes spectral clustering faster than standard SymNMF implementations but the randomized methods are able to bring SymNMF down to a more favorable runtime. A comment about this has been added to the main text.
    \item \textbf{Figure 1: How many trials with each method are run in this experiment?}
    Each method was run 10 times, and we have added a comment to the paper.
    \item \textbf{Line 746: “hyperparamter” should be “hyperparameter”}
    Done.
    \item \textbf{Figure 2: What are the projected gradient values in (b) and (d)? I don’t think this value is introduced until the appendix and is not referenced in the body of text describing this experiment.} We have added a more direct reference to the Appendix section where they are discussed.
    \item \textbf{Figure 2 caption: Is $\tau = 1/s$ correct? In the legend, it appears that this is defined differently for different trials.}
    Clarified in the figure caption.
    \item \textbf{Line 953: “The gradient of Eqn. Eq. (2.2) is given by...”}
    Fixed.
    \item \textbf{Figure 4, Table 4, Table 5: Should “LRA-...” be “LAI-...”? Additionally, are all these algorithm acronyms defined in the text? I don’t recognize SymNMF-HALS-1C for instance.} This is our mistake.  We have identified these typos/leftovers from previous versions and changed them to be consistent and clearer.
    \item \textbf{Lemma H.3: “... being true with probability $\delta$” should be “... with probability $\delta$.”}
    Done.
    \item \textbf{Theorem H.4: “Then for any $\epsilon > 0$ we have ...”}
    Done.
    \item \textbf{Theorem H.5: “... be a low-rank approximation of $\M{X}$...”}. Fixed.
\end{enumerate}




==> Theory_Section.tex <==
\section{Theoretical Results for Nonnegative Least Squares}
\label{sec:theory_nls}
We now explore some theoretical questions relevant to \cref{alg:lvs_nmf}.
Specifically we seek to answer two questions : 1) Can results for leverage score sampling for OLS problems be extended to NLS problems? and 2) What is the sample complexity of the Hybrid Sampling method from \cite{larsen2022sketching}?

%%%%%%%%%%%%%%%%%%%% START CLS %%%%%%%%%%%%%%%%%%%%%%
\input{LvS4CLS}
%%%%%%%%%%%%%%%%%%%% END CLS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% START Hybrid %%%%%%%%%%%%%%%%%%%%%%
\input{Hybrid_Sampling}
%%%%%%%%%%%%%%%%%%%% END Hybrid %%%%%%%%%%%%%%%%%%%%%%

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}
